RaPlace: Place Recognition for Imaging Radar using Radon Transform and Mutable Threshold

Due to the robustness in sensing, radar has been highlighted, overcoming harsh weather conditions such as fog and heavy snow. In this paper, we present a novel radar-only place recognition that measures the similarity score by utilizing Radon-transformed sinogram images and cross-correlation in frequency domain. Doing so achieves rigid transform invariance during place recognition, while ignoring the effects of radar multipath and ring noises. In addition, we compute the radar similarity distance using mutable threshold to mitigate variability of the similarity score, and reduce the time complexity of processing a copious radar data with hierarchical retrieval. We demonstrate the matching performance for both intra-session loop-closure detection and global place recognition using a publicly available imaging radar datasets. We verify reliable performance compared to existing stable radar place recognition method. Furthermore, codes for the proposed imaging radar place recognition is released for community.

==> note.tex <==
Camera Calibration of Thermal-Infrared Stereo Vision System
pg199 맨 윗줄에 circluar patten detecton이 checker board patten 찾는것보다 더 정확하다고 설명되있음

총 실행시간(ms)라는 내용 넣기

1. target geometry 위치
    method의 하나의 subsection으로
 
2. related work의 범위
 알고리즘을 완성시키는데 필요한 논문들은 method에서 다루고 calibration 관련 논문만 소개하자.
 
 3. 첫 페이지 그림 배치
 개발한 타겟이 첫 페이지에 나와주는게 임팩트 있을것 같은데 구조가 조금 난잡해 지는 문제
 ->두 그림 하나로 합치자
 
 4. introduction에 왜 point 기반이 아닌 conic을 사용했는지에 대한 설명 필요

----------------------------------------------------------

동일 시간이 흘렀을때 캘판과 우리 target의 boundary 변화를 figure로 나타내자
 

==> result_table.tex <==
%\begin{table*}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{c|c|cccc|c} 
%\hline
%\multirow{2}{*}{\textbf{Criteria}} & \multirow{2}{*}{\textbf{Approach}} &\multicolumn{4}{c|}{\textbf{Mulran Dataset}} & {\textbf{Oxford Dataset}}\\ 

% & & \textbf{DCC}  & \textbf{KAIST} & \textbf{Riverside} & \textbf{Sejong} & \textbf{2019-01-16 to 2019-01-18}\\ 
%\hline\hline
% & Raplace(Proposed) & \textbf{0.932} & \textbf{0.930} & \textbf{0.971} & \textbf{0.906} & %\textbf{0.949} \\
%\textbf{F1 Score} & Scan Context & 0.867 & 0.899 & 0.802 & 0.819 & 0.679\\
%& PointNetVLAD & 0.xxx & 0.xxx & 0.xxx & 0.xxx & 0.xxx\\
%\cline{1-7}
%& Raplace(Proposed) & \textbf{0.978} & \textbf{0.984} & \textbf{0.995} & \textbf{0.969} & %\textbf{0.959} \\
%\textbf{AUC} & Scan Context & 0.952 & 0.978 & 0.915 & 0.929 & 0.773\\
%& PointNetVLAD & 0.xxx & 0.xxx & 0.xxx & 0.xxx & 0.xxx  \\

%\end{tabular}}
%\caption{Global Localization Results.}\label{tab:gl_result}
%\end{table*}

\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|ccc}
\multicolumn{2}{c}{\textbf{Dataset}}                                                    & \textbf{Method} & \textbf{AUC}   & \textbf{F1 Score} \\ \hline\hline
\multicolumn{1}{c|}{\multirow{12}{*}{MulRan}} & \multirow{3}{*}{DCC}       & ScanContext     & 0.952          & 0.867             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.978} & \textbf{0.932}    \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{KAIST}     & ScanContext     & 0.978          & 0.899    \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.984} & \textbf{0.930}             \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{Riverside} & ScanContext     & 0.915          & 0.802             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.995} & \textbf{0.971}    \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{Sejong}    & ScanContext     & 0.929          & 0.819             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.969} & \textbf{0.906}    \\ \hline
\multicolumn{2}{c|}{\multirow{3}{*}{Oxford}}                     & ScanContext     & 0.773          & 0.679             \\  
\multicolumn{2}{c|}{}                                              & PointNetVlad    &                &                   \\ 
\multicolumn{2}{c|}{}                                          & RaPlace         & \textbf{0.959} & \textbf{0.949}    \\  \hline
\end{tabular}
}
\caption{Global Localization Results}\label{tab:gl_result}
\end{table}

==> result_table_comb.tex <==
\begin{table}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{cc|c|cc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset}}}                    & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Global Localization}}       \\
\multicolumn{2}{c|}{}                                                     &                                  & \multicolumn{1}{c}{\textbf{AUC}}   & \textbf{F1 Score} \\ \hline \hline
\multicolumn{1}{c|}{\multirow{8}{*}{MulRan}} & \multirow{2}{*}{DCC}       & SC                               & \multicolumn{1}{c}{0.952}          & 0.867             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.978}} & \textbf{0.932}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{KAIST}     & SC                               & \multicolumn{1}{c}{0.978}          & 0.899             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.984}} & \textbf{0.930}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Riverside} & SC                               & \multicolumn{1}{c}{0.915}          & 0.802             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.995}} & \textbf{0.971}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Sejong}    & SC                               & \multicolumn{1}{c}{0.929}          & 0.819             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.969}} & \textbf{0.906}    \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Oxford}} & \multirow{2}{*}{19-01-16}  & SC                               & \multicolumn{1}{c}{0.773}          & 0.679             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.959}} & \textbf{0.949}    \\ \hline
\end{tabular}
}
\caption{Global Localization Results}\label{tab:gl_result}
\end{table}
